Representation Transfer Learning via Multiple Pre-trained models for Linear Regression

In this paper, we consider the problem of learning a linear regression model on a data domain of interest (target) given few samples. To aid learning, we are provided with a set of pre-trained regression models that are trained on potentially different data domains (sources). Assuming a representation structure for the data generating linear models at the sources and the target domains, we propose a representation transfer based learning method for constructing the target model. The proposed scheme is comprised of two phases: (i) utilizing the different source representations to construct a representation that is adapted to the target data, and (ii) using the obtained model as an initialization to a fine-tuning procedure that re-trains the entire (over-parameterized) regression model on the target data. For each phase of the training method, we provide excess risk bounds for the learned model compared to the true data generating target model. The derived bounds show a gain in sample complexity for our proposed method compared to the baseline method of not leveraging source representations when achieving the same excess risk, therefore, theoretically demonstrating the effectiveness of transfer learning for linear regression.

==> app-p1.tex <==

\subsection{Proofs}

\subsubsection{Proof of Theorem~\ref{thm:low-dim-phase1} for Phase 1 Training}

We will first need to following lemma, the proof of which is provided later in the document.

\begin{lemma}[Multi-Source training guarantee] \label{lemm:multi_source_guarantee}
	With probability at least $1 - \frac{\delta}{5}$, we have:
	\begin{equation*}
		\sum_{i=1}^{m} \fverts{ \bfX_i ( \bfhB_i \bfhw_{i_0} - \bfB_i^{*} \bfw_{i_0}^{*} ) }_2^2 \leq \sigma^2 \left( km + kdm \log(\kappa n_s) + \log\left(\frac{1}{\delta}\right)  \right)
	\end{equation*}
	(See Section~\ref{app:low-dim} for proof.)
\end{lemma}



\begin{proof}
	We will first instantiate Lemma \ref{lemm:source_data}. We then instantiate Lemma~\ref{lemm:target_data} twice, once with $[ \bfhV \,\, -\bfV^{*}] $ and the other time with $ [\bfB_T^{*} \,\, -\bfV^{*}]$. Then we assume that the result from Lemma~\ref{lemm:multi_source_guarantee} holds. All these events happen together with probability at least $1 - \frac{2 \delta}{5}$.
	The expected error for the target distribution is given by:
	\begin{align*}
		\text{Err}(\{\bfhB_i \}_{i=1}^{m} , \bfw_T^{*})  &= \bbE_{\bfx \sim p_{T}} \left[ \bfx^{\top} \bfB_T^{*} \bfw_{T_0}^{*} -    \bfx^{\top} \bfhV \bfhw_T \right]^2  \\
		& = \fverts{\Sigma_T^{\nicefrac{1}{2}} \left(  \bfhV \bfhw_T -  \bfB_T^{*} \bfw_{T_0}^{*} \right)}_2^2  \\
		& \lesssim \fverts{\Sigma_T^{\nicefrac{1}{2}} \left(  \bfhV \bfhw_T -  \bfV^{*} \bfw_T^{*} \right)}_2^2 + \fverts{\Sigma_T^{\nicefrac{1}{2}} \left(   \bfB_T^{*} \bfw_{T_0}^{*} -  \bfV^{*} \bfw_T^{*} \right)}_2^2  \\
		& \stackrel{As.~\ref{assump:source_target_map}}{\leq} \fverts{\Sigma_T^{\nicefrac{1}{2}} \left(   \bfhV \bfhw_T -  \bfV^{*} \bfw_T^{*} \right)}_2^2 + \epsilon^2 \\
		& \stackrel{Lem.~\ref{lemm:target_data}}{\lesssim} \frac{1}{n_T} \fverts{ \bfX_T \left(  \bfhV \bfhw_T -  \bfV^{*} \bfw_T^{*} \right)}_2^2 + \epsilon^2 \\
		& = \frac{1}{n_T} \fverts{  \bfP_{\bfX_T  \bfhV} \bfy_T -  \bfX_T \bfV^{*} \bfw_T^{*} }_2^2 + \epsilon^2 \\
		& \lesssim \frac{1}{n_T} \fverts{ \bfP_{\bfX_T  \bfhV} (\bfX_T \bfV^{*} \bfw_T^{*} + \bfz_T ) - \bfX_T \bfV^{*} \bfw_T^{*} )}_2^2 \\
		& \qquad + \frac{1}{n_T}	\fverts{  \bfP_{\bfX_T  \bfhV} (\bfX_T \bfB_T^{*} \bfw_{T_0}^{*} - \bfX_T \bfV^{*} \bfw_T^{*})  }_2^2 + \epsilon^2 \\
		\intertext{Using the fact that $\Vert \bfP_{\bfX_T \bfhV}  \Vert_2 \leq 1 $ and using Lemma~\ref{lemm:target_data} we have:}
		& \stackrel{As.~\ref{assump:source_target_map}, Lem.~\ref{lemm:target_data}}{\lesssim} \frac{1}{n_T} \fverts{ \bfP_{\bfX_T  \bfhV} (\bfX_T \bfV^{*} \bfw_T^{*} + \bfz_T ) - \bfX_T \bfV^{*} \bfw_T^{*} )}_2^2 + \epsilon^2 \\
		& \lesssim \frac{1}{n_T} \fverts{ \bfP^{\perp}_{\bfX_T  \bfhV} \bfX_T \bfV^{*} \bfw_T^{*}}_2^2 + \epsilon^2 + \frac{1}{n_T} \fverts{\bfP_{\bfX_T  \bfhV} \bfz_T }_2^2
	\end{align*}
	We can take the expectation over the distribution of $\bfw_T^{*}$ and use Assumption~\ref{assump:target_task_dist} to yield:
	\begin{align} \label{eq:multi_1}
		\bbE_{\bfw_T^{*}} [\text{Err}(\bfhV , \bfw_T^{*})] \lesssim \frac{1}{n_Tl} \fverts{ \bfP^{\perp}_{\bfX_T  \bfhV} \bfX_T \bfV^{*} }_F^2 + \epsilon^2 + \frac{1}{n_T} \fverts{\bfP_{\bfX_T \bfhV} \bfz_T }_2^2
	\end{align}
	We now make use of the following lemma, proved later in the document which provides a bound for the first term in \eqref{eq:multi_1}.
	\begin{lemma}[Target guarantee (for multi-source)] \label{lemm:multi_target_gurantee}
		Assuming the results in Lemma~\ref{lemm:source_data}, Lemma~\ref{lemm:target_data} (with $\bfB = [ \bfhV \quad - \bfV^{*} ]$) and lemma~\ref{lemm:multi_source_guarantee} hold, we then have:
		\begin{align*}
			\fverts{ \bfP^{\perp}_{\bfX_T  \bfhV} \bfX_T \bfV^{*} }_F^2 & \lesssim \frac{n_T}{c n_s\sigma_l^2(\bfW^{*}) } \sigma^2 \left( km + kdm \log(\kappa n_s) + \log\left(\frac{1}{\delta}\right)  \right) 
		\end{align*}
	\end{lemma} 
	Substituting the result from Lemma~\ref{lemm:multi_target_gurantee} in \eqref{eq:multi_1} and using $\sigma_l^2(\bfW^{*}) \geq \frac{m}{l}$, the following bound holds with probability at least $1 - \frac{2 \delta}{5}$:
	\begin{align*}
		\bbE_{\bfw_T^{*}} [\text{Err}(\bfhV , \bfw_T^{*})]& \lesssim \frac{1}{c  n_sm } \sigma^2 \left( km + kdm \log(\kappa n_s) + \log\left(\frac{1}{\delta}\right)  \right) + \epsilon^2 \\
		& \qquad  + \frac{1}{n_T} \fverts{\bfP_{\bfX_T  \bfhV } \bfz_T }_2^2 
	\end{align*}
	Finally, the last term in above can be bounded by using a concentration inequality for $\chi^2$-squared distribution. In particular, with probability at least $1 - \frac{3\delta}{5}$ we have $\verts{\bfP_{\bfX_T  \bfhV} \bfz_T }_2^2 \lesssim \sigma^2 (q + \log(\nicefrac{1}{\delta})) $. Thus the following bound holds on $\bbE_{\bfw_T^{*}} [\text{Err}( \bfhB_S , \bfw_T^{*})]$ with probability at least $1 - \delta$:
	
	\begin{align*}
		\bbE_{\bfw_T^{*}} [\text{Err}(\bfhV , \bfw_T^{*})] & \lesssim \frac{1}{c n_sm } \sigma^2 \left( km + kdm \log(\kappa n_s) + \log\left(\frac{1}{\delta}\right)  \right) + \epsilon^2  + \frac{1}{n_T} \sigma^2 (q + \log(\nicefrac{1}{\delta})) \\
		& = \sigma^2 \left[\frac{1}{c n_sm }  \log\left(\frac{1}{\delta}\right)  +  \left(\frac{kd \log(\kappa n_s) + k}{c n_s}\right)  + \frac{1}{n_T} (q + \log(\nicefrac{1}{\delta}))\right]  + \epsilon^2 
	\end{align*}
	
\end{proof}





\begin{proposition} \label{prop:mat_cols}
	Consider matrices $\bfA \in \bbR^{a \times b}$  and $\bfB \in \bbR^{b \times c} $. Then for any $\bfu \in \bbR^{a}$, we have:
	\begin{equation*}
		\Vert \bfP^{\perp}_{\bfA } \bfu \Vert_2^2 \leq \Vert \bfP^{\perp}_{\bfA \bfB} \bfu \Vert_2^2
	\end{equation*} 
\end{proposition}
\begin{proof}
	For given $\bfA \in \bbR^{a \times b}$ and $\bfB \in \bbR^{b \times c}$ and $\bfu \in \bbR^{a}$, we have:
	\begin{align*}
		\Vert \bfP^{\perp}_{\bfA } \bfu \Vert_2^2 & = \min_{\mathbf{r} \in \bbR^{b}} \Vert \bfA \mathbf{r} - \bfu \Vert_2^2 \\
		& \leq \min_{\mathbf{r} \in \mathcal{C}(\bfB)} \Vert \bfA \mathbf{r} - \bfu \Vert_2^2 \\
		& = \min_{\mathbf{s} \in \bbR^{c}} \Vert \bfA \bfB \mathbf{s} - \bfu \Vert_2^2 \\
		& = \Vert \bfP^{\perp}_{\bfA \bfB} \bfu \Vert_2^2
	\end{align*}
\end{proof}




%%%---------------------


\subsubsection{Proof for Theorem~\ref{thm:low-dim-phase2} for Phase 2 training} \label{subsubsec:low-dim-phase2-proof}

We define $\bfP_{\parallel} = \bfX^{\top} (\bfX\bfX^{\top})^{-1}\bfX$ as projection matrix on the rowspace of matrix $\bfX$ and $\bfP_{\perp} = \bfI - \bfP_{\parallel}$. (Here, $\bfX$ refers to the target matrix $\bfX_T$ unless stated otherwise.) \\
We first note the following result which establishes where the Gradient Descent solution converges to, the proof of which is given in Section~\ref{app:low-dim}
\begin{lemma} \label{lemm:gradient-descent-soln}
	Under the assumptions stated in Section~\ref{assump:low-dim-phase2}, performing gradient descent on the objective \eqref{eq:fine-tune_obj} with the initialization $\btheta^{(0)} := \btheta_{T_0}$ and learning rate $\eta$, yields the solution:
	\begin{equation*}
		\btheta_{GD} := \btheta^{(\infty)} =  \bfP_{\parallel}\btheta_T^{*} + \bfP_{\perp} \btheta_{T_0} + \bfX^{\top}(\bX \bX^{\top})^{-1} \boldsymbol{\varepsilon}
	\end{equation*}
\end{lemma}

We now use the solution of the gradient descent $\btheta_{GD}$ derived in Lemma~\ref{lemm:gradient-descent-soln} and find the excess population risk. The excess risk is given by:
\begin{align*}
	\text{Err}(\btheta_{GD},\btheta_T^{*}) & = \bbE_{\bx \sim p_T} (\bx^{\top} \btheta_T^{*} - \bx^{\top} \btheta_{GD}  )^2 \\
	& =  \bbE_{\bx \sim p_T} \text{Tr} [(\btheta_{T}^{*} - \btheta_{GD})^{\top}\bx \bx^{\top}(\btheta_{T}^{*} - \btheta_{GD})] \\
	& = \verts{\Sigma_T^{\nicefrac{1}{2}}(\btheta_{T}^{*} - \btheta_{GD})}_2^2
\end{align*}
Substituting the value of $\btheta_{GD}$ from Lemma~\ref{lemm:gradient-descent-soln} we get:
\begin{align} \label{eq:interim5}
	\text{Err}(\btheta_{GD},\btheta_T^{*}) \leq 2 \verts{\Sigma_T^{\nicefrac{1}{2}} \bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})  }_2^2 + 2\verts{ \Sigma_T^{\nicefrac{1}{2}} \bfX^{\top}(\bX \bX^{\top})^{-1} \boldsymbol{\varepsilon} }_2^2
\end{align}
Note that the second term in above can be bounded by using a concentration bound on the $\chi-$squared distribution. We focus on the first term for now. We have
\begin{align} \label{eq:interim6}
	\verts{\Sigma_T^{\nicefrac{1}{2}} \bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})  }_2^2
	& = (\btheta_T^{*} - \btheta_{T_0})^{\top} \bfP_{\perp}^{\top} \Sigma_T \bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})  \notag \\
	& = (\btheta_T^{*} - \btheta_{T_0})^{\top} \bfP_{\perp}^{\top} \left(\Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX \right) \bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})\notag \\
	& = \left\Vert \left(\Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX \right)^{\nicefrac{1}{2}} \bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})  \right\Vert_2^2 \notag \\
	& \leq \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX  \right\Vert_2 \verts{\bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})}_2^2
\end{align}
The second term in \eqref{eq:interim6} can be bounded by $\verts{\bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})}_2^2 \leq \verts{(\btheta_{T}^{*} - \btheta_{T_0})}_2^2$ by noting that $\bfP_{\perp} \leq 1$. We can also use the David-Kahn $\sin-\theta$ theorem to provide a bound for this term as done in \cite{shachaf2021theoretical}. \footnote{ Consider the SVD of $\Sigma_T = \bfV \bLambda \bfV^{\top} $ and $\bfX = \bftU \btGamma \bftV^{\top}$. Since $\bfX \in \bbR^{n_T \times d}$, $\btGamma$ has its last $d-n_T$ entries as 0. It can be checked that $\bfP_{\parallel} = \bfX^{\top}(\bfX\bfX^{\top})^{-1} \bfX = \bfI - \bftV_{>n_T} \bftV_{>n_T}^{\top} $ where $\bftV_{>n_T}$ denotes the submatrix of $\bftV$ containing columns from $n_T+1$ to $d$. Thus, $P_{\perp} = \bftV_{>n_T} \bftV_{>n_T}^{\top}$. We now note that for any $c \in [d]$, we have:
	\begin{align*}
		\verts{\bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})}_2^2 &= \Vert \bftV_{>n_T}^{\top} (\btheta_{T}^{*} - \btheta_{T_0}) \Vert_2^2 \\
		& = \Vert \bftV_{>n_T}^{\top} \bfV \bfV^{\top}  (\btheta_{T}^{*} - \btheta_{T_0}) \Vert_2^2 \\
		& \leq  2\verts{\bftV_{>n_T}^{\top} \bfV_{>c} }_2^2  \verts{\bfV_{>c}^{\top}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2 + 2\verts{\bftV_{>n_T}^{\top} \bfV_{\leq c} }_2^2  \verts{\bfV_{ \leq c}^{\top}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2\\
		\intertext{Using the fact $\verts{\bftV_{>n_T}^{\top} \bfV_{>c} }_2^2 \leq \verts{\bfV^{\top}_{>n_T}}_2^2 \verts{ \bfV_{>c} }_2^2 = \verts{\bfV_{>n_T}}_2^2 \verts{ \bfV_{>c} }_2^2 \leq 1$, we get:}
		& \leq  2 \verts{\bfV_{>c}^{\top}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2 + 2\verts{\bftV_{>n_T}^{\top} \bfV_{\leq c} }_2^2  \verts{\bfV_{ \leq c}^{\top}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2\\
		\intertext{Using the result from \cite{shachaf2021theoretical}[Lemma 1.4] to bound $\verts{\bftV_{>n_T}^{\top} \bfV_{\leq c} }_2^2$ which uses the David-Kahn sin-$\theta$ theorem, we get}
		& \leq 2 \verts{\bfV_{>c}^{\top}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2 + \frac{2}{\lambda^2_c}  \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top} \bfX \right\Vert_2^2   \verts{\bfV_{ \leq c}^{\top}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2\\
		& = 2\verts{\bfP_{>c}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2 + \frac{2}{\lambda^2_c}  \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top} \bfX \right\Vert_2^2 \verts{ \bfP_{\leq c} (\btheta_{T}^{*} - \btheta_{T_0})}_2^2
	\end{align*}
	Substituting this in \eqref{eq:interim6} yields:
	\begin{align*}
		\verts{\Sigma_T^{\nicefrac{1}{2}} \bfP_{\perp}(\btheta_{T}^{*} - \btheta_{T_0})  }_2^2 \leq 2 \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX  \right\Vert_2  \verts{\bfP_{>c}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2 + \frac{2}{\lambda^2_c} \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX  \right\Vert_2^3 \verts{ \bfP_{\leq c} (\btheta_{T}^{*} - \btheta_{T_0})}_2^2
	\end{align*}
	Substituting the above expression in \eqref{eq:interim5} finally yields:
	\begin{align*} 
		\text{Err}(\btheta_{GD},\btheta_T^{*})& \leq 4 \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX  \right\Vert_2  \verts{\bfP_{>c}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2 + \frac{4}{\lambda^2_c} \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX  \right\Vert_2^3 \verts{ \bfP_{\leq c} (\btheta_{T}^{*} - \btheta_{T_0})}_2^2 \notag \\
		& \quad + 2\verts{ \Sigma_T^{\nicefrac{1}{2}} \bfX^{\top}(\bX \bX^{\top})^{-1} \boldsymbol{\varepsilon} }_2^2
	\end{align*}
	This can be useful in a setting where we know that $\verts{\bfP_{>c}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2$ is much smaller compared to $\verts{\bfP_{\leq c}  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2$.
}

We thus finally get the bound:
\begin{align} \label{eq:interim7}
	\text{Err}(\btheta_{GD},\btheta_T^{*})& \leq 2 \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX  \right\Vert_2  \verts{  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2  + 2\verts{ \Sigma_T^{\nicefrac{1}{2}} \bfX^{\top}(\bX \bX^{\top})^{-1} \boldsymbol{\varepsilon} }_2^2
\end{align}

We now provide a bound for the second term in \eqref{eq:interim7}. It can be seen that
\begin{align*} 
	\verts{ \Sigma_T^{\nicefrac{1}{2}} \bfX^{\top}(\bX \bX^{\top})^{-1} \boldsymbol{\varepsilon} }_2^2 & =
	\boldsymbol{\varepsilon}^{\top} (\bfX \bX^{\top})^{-1}  \bX \Sigma_T \bfX^{\top}(\bX \bX^{\top})^{-1} \boldsymbol{\varepsilon}
	\intertext{From Lemma 9 in \cite{bartlett2020benign}, we can get a high probability bound (probability $>1 - e^{-t}$) on this term for some $t >0$ as}
	& \leq (4t+2) \sigma^2 \text{Tr}\left( (\bfX \bX^{\top})^{-1}  \bX \Sigma_T \bfX^{\top}(\bX \bX^{\top})^{-1} \right) 
\end{align*}
To bound the trace term, we use Lemma 13 and Lemma 18 from \cite{bartlett2020benign}. For universal constant $b,c \geq1$ and $k^{*} := \min \{k\geq 0 : r_k(\Sigma_T) \geq bn\}$, then 
\begin{align*}
	\textbf{Tr}\left( (\bfX \bX^{\top})^{-1}  \bX \Sigma_T \bfX^{\top}(\bX \bX^{\top})^{-1} \right) \leq c \left( \frac{k^{*}}{bn} + \frac{bn}{ R_{k^{*}}(\Sigma_T) } \right)
\end{align*}
where $r_k(\Sigma_T) = \frac{\Sigma_{i>k} \lambda_i}{\lambda_{k+1}} $, $R_{k^{*}}(\Sigma_T) = \frac{(\Sigma_{i>k} \lambda_i)^2}{\Sigma_{i>k} \lambda_i^2} $. A discussion on these `Effective Ranks' can be found in \cite{bartlett2020benign}.
Substituting the value of $t = \log\left(\frac{2}{\delta}\right)$
Plugging the bound from \eqref{eq:interim11} in \eqref{eq:interim7}, we can finally claim that the following holds with probability at least $1-\frac{\delta}{2}$:
\begin{align*}
	\text{Err}(\btheta_{GD},\btheta_T^{*}) & \lesssim  \left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top}\bfX  \right\Vert_2  \verts{  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2  + c \sigma^2 \log\left(\frac{1}{\delta}\right)  \left( \frac{k^{*}}{bn} + \frac{bn}{ R_{k^{*}}(\Sigma_T) } \right)
\end{align*}
The covariance approximation error in the first term of above can be bounded by the result in \cite{koltchinskii2017concentration}[Theorem 9]. This yields the following bound on the approximation with probability at least $1- e^{-\delta_1}$ over the choice of data matrix $\bfX$ for some constant $u >0$ and $\delta_1 >1$
\begin{align*}
	\left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top} \bfX \right\Vert_2 \leq u \lambda_1 \max \left\{ \sqrt{\frac{\sum_{i=1}^{d} \lambda_i }{n_T \lambda_1}},\frac{\sum_{i=1}^{d} \lambda_i }{n_T \lambda_1}, \sqrt{\frac{\delta_1}{n_T}},\frac{\delta_1}{n_T}   \right\}
\end{align*}

Substituting $\delta_1 = \log \left(\frac{2}{\delta} \right)$, we get with probability at least $1 - \frac{\delta}{2}$ that

\begin{align*}
	\left\Vert \Sigma_T - \frac{1}{n_T} \bfX^{\top} \bfX \right\Vert_2 \leq u \lambda_1 \max \left\{ \sqrt{\frac{\sum_{i=1}^{d} \lambda_i }{n_T \lambda_1}},\frac{\sum_{i=1}^{d} \lambda_i }{n_T \lambda_1}, \sqrt{\frac{1}{n_T} \log\left(\frac{1}{\delta}\right) },\frac{1}{n_T} \log \left(\frac{1}{\delta}\right)   \right\}
\end{align*}


%%_---------------------------------------

\subsubsection{Proof of Proposition~\ref{prop:low-dim-combined}}

Consider the result from Theorem~\ref{thm:low-dim-phase2} for the bound on the excess risk after Phase 2 training given by:
\begin{align*}
	\text{Err}(\btheta_{GD},\btheta_T^{*}) & \lesssim  \left\Vert \Sigma_T - \frac{1}{n_{T_2}} \bfX^{\top}\bfX  \right\Vert_2  \verts{  (\btheta_{T}^{*} - \btheta_{T_0})}_2^2  + c \sigma^2 \log\left(\frac{1}{\delta}\right)  \left( \frac{k^{*}}{bn_{T_2}} + \frac{bn_{T_2}}{ R_{k^{*}}(\Sigma_T) } \right)
\end{align*}
Denote the eigenvalues of covariance matrix of the target data as $\{ \lambda_i\}_{i=1}^{d}$, with $\lambda_1 \geq \hdots \lambda_d$, we then have:
\begin{align*}
	\text{Err}(\btheta_{GD},\btheta_T^{*}) \lesssim \left\Vert \Sigma_T - \frac{1}{n_{T_2}} \bfX^{\top}\bfX  \right\Vert_2  \frac{1}{\lambda_d} \verts{ \Sigma_T (\btheta_{T}^{*} - \btheta_{T_0})}_2^2  + c \sigma^2 \log\left(\frac{1}{\delta}\right)  \left( \frac{k^{*}}{bn_{T_2}} + \frac{bn_{T_2}}{ R_{k^{*}}(\Sigma_T) } \right)
\end{align*}
where $r_k(\Sigma_T) = \frac{\Sigma_{i>k} \lambda_i}{\lambda_{k+1}} $, $R_{k^{*}}(\Sigma_T) = \frac{(\Sigma_{i>k} \lambda_i)^2}{\Sigma_{i>k} \lambda_i^2} $.	Here, constant $b>1$ and $k^{*} = \min \{ k \geq 0: r_k(\Sigma) \geq bn \}$.
The covariance estimation term can be bounded by $
\left\Vert \Sigma_T - \frac{1}{n_{T_2}} \bfX^{\top} \bfX \right\Vert_2 \leq u \lambda_1 \max \left\{ \sqrt{\frac{\sum_{i=1}^{d} \lambda_i }{n_{T_2} \lambda_1}},\frac{\sum_{i=1}^{d} \lambda_i }{n_{T_2} \lambda_1}, \sqrt{\frac{1}{n_{T_2}} \log\left(\frac{1}{\delta}\right) },\frac{1}{n_{T_2}} \log \left(\frac{1}{\delta}\right)   \right\}
$ with probability at least $1 - \frac{\delta}{2}$. 
We now substitute the value of $\verts{ \Sigma_T (\btheta_{T}^{*} - \btheta_{T_0})}_2^2$ from Theorem~\ref{thm:low-dim-phase1} (as $\btheta_{T_0} = \bfhV \bfhw_T$ which was obtained by using $n_{T_1}$ target samples). Thus the final bound after Phase 1 and Phase 2 training, after taking the expectation w.r.t the target model $\btheta_{T}^{*}$, is given by:
\begin{align*}
	\bbE \text{Err}(\btheta_{GD},\btheta_T^{*}) & \lesssim \left\Vert \Sigma_T - \frac{1}{n_{T_2}} \bfX^{\top} \bfX \right\Vert_2 \frac{1}{\lambda_d} \left(\sigma^2 \left[\frac{1}{c n_sm}  \log\left(\frac{1}{\delta}\right)  +  \left(\frac{kd \log(\kappa n_s) + k}{c n_s}\right)  + \frac{1}{n_{T_1}} ( q  + \log(\nicefrac{1}{\delta}))\right]  + \epsilon^2\right) \\
	& \qquad + c \sigma^2 \log\left(\frac{1}{\delta}\right)  \left( \frac{k^{*}}{bn_{T_2}} + \frac{bn_{T_2}}{ R_{k^{*}}(\Sigma_T) } \right) 
\end{align*}
where $u,c$ are universal constants. We can simplify this as (assuming $\frac{r_0(\Sigma_T) }{n_{T_2}} \geq \frac{1}{n_{T_2}} \log \left(\frac{1}{\delta}\right) \geq 1$ as we have a few target samples)
\begin{align*}
	\bbE \text{Err}(\btheta_{GD},\btheta_T^{*}) & \leq \frac{u \lambda_1 }{\lambda_d}  \frac{r_0(\Sigma_T) }{n_{T_2}}   \left(\frac{\sigma^2 }{n_{T_1}} ( q  + \log(\nicefrac{1}{\delta})) + \epsilon^2 \right) + c \sigma^2 \log\left(\frac{1}{\delta}\right)  \left( \frac{k^{*}}{bn_{T_2}} + \frac{bn_{T_2}}{ R_{k^{*}}(\Sigma_T) } \right)  \\
	& \qquad + \frac{u \lambda_1 \sigma^2 }{\lambda_d} \frac{r_0(\Sigma_T) }{n_{T_2}} \left(\frac{1}{c n_sm}  \log\left(\frac{1}{\delta}\right)  +  \left(\frac{kd \log(\kappa n_s) + k}{c n_s}\right)\right)
\end{align*}








==> headers_new.tex <==
\usepackage[T1]{fontenc}
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
%\usetikzlibrary{snakes}
\usepackage{cite}
\usepackage{graphicx}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{mdwtab}
\usepackage{eqparbox}
\usepackage{fixltx2e}
\usepackage{url}
\usepackage{pgf}
\usepackage{lipsum}
\usepackage{multirow}
%\usepackage{subcaption}
%\usepackage{subfigure}
%\usepackage[cmex10]{amsmath}
\usepackage{amsfonts,amssymb,amsthm}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{algorithmic}
\usepackage{bm}
\usepackage{bbm}
\usepackage{booktabs}
\usepackage{etoolbox}
\usepackage{makecell}
\usepackage{nicefrac}
\usepackage{textcomp}
\usepackage{stmaryrd}
\usepackage{mathrsfs}
\usepackage{paralist}
\usepackage{comment}
\usepackage{lmodern}

\usepackage[font=footnotesize,labelsep=space,labelfont=bf]{caption}

\usepackage[colorlinks=true, citecolor=burntumber, linkcolor = bluepigment ,urlcolor=blue, pagebackref=false]{hyperref}
%\usepackage{url}

\hyphenation{op-tical net-works semi-conduc-tor}

%\usepackage[pdftex,bookmarks=true,pdfstartview=FitH,colorlinks,linkcolor=blue,filecolor=blue,citecolor=blue,urlcolor=blue,pagebackref=false]{hyperref}
%    \urlstyle{sf}

%\usepackage[draft]{hyperref}
%\usepackage{url}


\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother



\newtheorem{theorem}{Theorem}%[chapter]
\newtheorem*{theorem*}{Theorem}
\newtheorem{definition}{Definition}%[chapter]
\newtheorem{lemma}{Lemma}%[chapter]
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim}{Claim}%[chapter]
\newtheorem{corollary}{Corollary}%[chapter]
\newtheorem*{cor*}{Corollary}
\newtheorem{remark}{Remark}%[chapter]
\newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}%[chapter]
\newtheorem*{fact*}{Fact}%[chapter]

\newcommand{\TODO}[1]{{{\color{red}#1}}}
\newcommand{\CHECK}[1]{{{\color{blue}#1}}}
\newcommand{\CHECKM}[1]{{{\color{magenta}#1}}}

\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}}

\newcommand{\WZ}{\text{WZ}}
\newcommand{\PS}{\text{PS}}
\newcommand{\AS}{\text{AS}}
\newcommand{\EQ}{\text{EQ}}
\newcommand{\GK}{\text{GK}}
\newcommand{\image}{\text{image}}

%\newcommand{\Algorithmref}[1]{\namedref{Algorithm}{algo:#1}}
%\newcommand{\Chapterref}[1]{\namedref{Chapter}{chap:#1}}
%\newcommand{\Sectionref}[1]{\namedref{Section}{sec:#1}}
%\newcommand{\Subsectionref}[1]{\namedref{Section}{subsec:#1}}
%\newcommand{\Subsubsectionref}[1]{\namedref{Section}{subsubsec:#1}}
%\newcommand{\Appendixref}[1]{\namedref{Appendix}{app:#1}}
%\newcommand{\Theoremref}[1]{\namedref{Theorem}{thm:#1}}
%\newcommand{\Corollaryref}[1]{\namedref{Corollary}{cor:#1}}
%\newcommand{\Propositionref}[1]{\namedref{Proposition}{prop:#1}}
%\newcommand{\Conjectureref}[1]{\namedref{Conjecture}{conj:#1}}
%\newcommand{\Definitionref}[1]{\namedref{Definition}{defn:#1}}
%\newcommand{\Lemmaref}[1]{\namedref{Lemma}{lem:#1}}
%\newcommand{\Remarkref}[1]{\namedref{Remark}{remark:#1}}
%\newcommand{\Claimref}[1]{\namedref{Claim}{claim:#1}}
%\newcommand{\Factref}[1]{\namedref{Fact}{fact:#1}}
%\newcommand{\Tableref}[1]{\namedref{Table}{tab:#1}}
%\newcommand{\Figureref}[1]{\namedref{Figure}{fig:#1}}
%\newcommand{\Equationref}[1]{\namedref{Equation}{eq:#1}}
%\newcommand{\Footnoteref}[1]{\namedref{Footnote}{foot:#1}}
%\newcommand{\Pageref}[1]{\hyperref[#1]{page~\pageref*{#1}}}



%%%%
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}


%\definecolor{darkred}{rgb}{0.5, 0, 0} 
%\definecolor{darkblue}{rgb}{0,0,0.5} 
%\hypersetup{
%    colorlinks=true,
%    linkcolor=darkred,
%    citecolor=darkblue,
%    urlcolor=darkblue   
%}


\renewcommand{\ij}{\ensuremath{\vec{ij}}\xspace}
\newcommand{\ji}{\ensuremath{\vec{ji}}\xspace}
\newcommand{\Rplus}{\ensuremath{\mathbb{R}_+}\xspace}

\newcommand{\PinextA}{\ensuremath{\mathrm{next}^A_\Pi}\xspace}
\newcommand{\PinextB}{\ensuremath{\mathrm{next}^B_\Pi}\xspace}
\newcommand{\PioutA}{\ensuremath{\mathrm{out}^A_\Pi}\xspace}
\newcommand{\PioutB}{\ensuremath{\mathrm{out}^B_\Pi}\xspace}
\newcommand{\Piout}{\ensuremath{\mathrm{out}_\Pi}\xspace}
\newcommand{\Pipr}[1]{\ensuremath{\mathrm{Pr}_\Pi[#1]}\xspace}
\newcommand{\Pileft}{\ensuremath{\Pi^{(0)}}\xspace}
\newcommand{\Pileftpr}[1]{\ensuremath{\mathrm{Pr}_{\Pileft}[#1]}\xspace}
\newcommand{\fleft}{\ensuremath{f^{(0)}}\xspace}
\newcommand{\Xleft}{\ensuremath{\X^{(0)}}\xspace}
\newcommand{\rholeft}{\ensuremath{\rho^{(0)}}\xspace}
\newcommand{\sigmaleft}{\ensuremath{\sigma^{(0)}}\xspace}
\newcommand{\fright}{\ensuremath{f^{(1)}}\xspace}

\newcommand{\Pizeroout}{\ensuremath{\mathrm{out}_{\Pi_0}}\xspace}

\newcommand{\balpha}{\ensuremath{{\bf \alpha}}\xspace}
\newcommand{\bzero}{\ensuremath{{\bf 0}}\xspace}
\newcommand{\RI}{\ensuremath{RI}\xspace}
\newcommand{\supp}{\ensuremath{\textsf{supp}}\xspace}
\newcommand{\ba}{\ensuremath{{\bf a}}\xspace}
\newcommand{\bb}{\ensuremath{{\bf b}}\xspace}
\newcommand{\doublebarbx}{\ensuremath{\bar{\bar{{\bf x}}}}\xspace}
\newcommand{\btb}{\ensuremath{\tilde{\bf b}}\xspace}
\newcommand{\bc}{\ensuremath{{\bf c}}\xspace}
\newcommand{\bd}{\ensuremath{{\bf d}}\xspace}
\newcommand{\be}{\ensuremath{{\bf e}}\xspace}
\newcommand{\bhe}{\ensuremath{\hat{\bf e}}\xspace}
\newcommand{\bte}{\ensuremath{\tilde{\bf e}}\xspace}
\newcommand{\bbf}{\ensuremath{{\bf f}}\xspace}
\newcommand{\btf}{\ensuremath{\tilde{\bf f}}\xspace}
\newcommand{\bg}{\ensuremath{{\bf g}}\xspace}
\newcommand{\br}{\ensuremath{{\bf r}}\xspace}
\newcommand{\btr}{\ensuremath{\tilde{\bf r}}\xspace}
\newcommand{\bx}{\ensuremath{{\bf x}}\xspace}
\newcommand{\bp}{\ensuremath{{\bf p}}\xspace}
\newcommand{\barbp}{\ensuremath{\overline{\mathbf{p}}}\xspace}
\newcommand{\bwx}{\ensuremath{\widehat{\bf x}}\xspace}
\newcommand{\btx}{\ensuremath{\widetilde{\bf x}}\xspace}
\newcommand{\blx}{\ensuremath{\overline{\bf x}}\xspace}
\newcommand{\by}{\ensuremath{{\bf y}}\xspace}
\newcommand{\bty}{\ensuremath{\widetilde{\bf y}}\xspace}
\newcommand{\bz}{\ensuremath{{\bf z}}\xspace}
\newcommand{\bs}{\ensuremath{{\bf s}}\xspace}
\newcommand{\bts}{\ensuremath{\tilde{\bf s}}\xspace}
\newcommand{\bw}{\ensuremath{{\bf w}}\xspace}
\newcommand{\btw}{\ensuremath{\widetilde{\bf w}}\xspace}
\newcommand{\bu}{\ensuremath{{\bf u}}\xspace}
\newcommand{\bv}{\ensuremath{{\bf v}}\xspace}
\newcommand{\nr}{\ensuremath{{n_r}}\xspace}
\newcommand{\nc}{\ensuremath{{n_c}}\xspace}
\newcommand{\bA}{\ensuremath{{\bf A}}\xspace}
\newcommand{\bE}{\ensuremath{{\bf E}}\xspace}
\newcommand{\bI}{\ensuremath{{\bf I}}\xspace}
\newcommand{\bF}{\ensuremath{\boldsymbol{F}}\xspace}
\newcommand{\bT}{\ensuremath{{\bf T}}\xspace}
\newcommand{\calS}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\bS}{\ensuremath{{\bf S}}\xspace}
\newcommand{\btS}{\ensuremath{\tilde{\bf S}}\xspace}
\newcommand{\bX}{\ensuremath{{\bf X}}\xspace}
\newcommand{\bV}{\ensuremath{{\bf V}}\xspace}
\newcommand{\bW}{\ensuremath{{\bf W}}\xspace}
\newcommand{\btX}{\ensuremath{\widetilde{\bf X}}\xspace}
\newcommand{\bhX}{\ensuremath{\widehat{\bf X}}\xspace}
\newcommand{\blX}{\ensuremath{\overline{\bf X}}\xspace}
\newcommand{\bxi}{\ensuremath{\boldsymbol{\xi}}\xspace}
\newcommand{\out}[1]{\ensuremath{\Pi^{\text{out}}_{#1}}\xspace}
\newcommand{\A}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\B}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\C}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\bbE}{\ensuremath{\mathbb{E}}\xspace}
\newcommand{\bbN}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\bbR}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\calO}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\I}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\calP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Y}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\Z}{\ensuremath{\mathcal{Z}}\xspace}
\newcommand{\U}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\V}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\W}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\M}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\N}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\setS}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\E}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\G}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\R}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\T}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\bbZ}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\equi}{\ensuremath{\triangleleft}\xspace}
\newcommand{\mx}{\ensuremath{\mathsf{Max}}\xspace}
\newcommand{\MaxTerm}{\ensuremath{\mathrm{MaxTerm}}\xspace}
\newcommand{\tmx}{\ensuremath{\mathsf{\widetilde{Max}}}\xspace}

\newcommand{\jbar}{\ensuremath{{\bar{\jmath}}}\xspace}
\newcommand{\zz}[1]{{\color{gray}\ensuremath{z_{#1}}}\xspace}



\newcommand{\twobythreetable}[8]{%
\protect{\begin{tabular}{|c|ccc|}\hline & $#1_1$ & $#1_2$ & $#1_3$  \\\hline $#2_1$ & #3 & #4 & #5 \\ $#2_2$ & #6 & #7 & #8\\\hline\end{tabular}}}


\renewcommand{\paragraph}[1]{\smallskip\noindent{\bf #1}~}


==> p1_low-dim-rep.tex <==
\allowdisplaybreaks
{
	
	

	We work with following setting:
	\begin{itemize}
		\item The dimension of the input vector $\bfx_i$ is $d$
		\item The dimension of vector $\bfw_{i_0}$ is $k$, with $k \ll d$.
		\item $\{\bfB_i^{*}\} \subseteq \mathbb{R}^{d \times k}$. % It is assumed the columns of the representation matrices $\{\bfB_i^{*}\}_{i=1}^{m}$ are orthonormal, i.e., $(\bfB^{*}_i)^{\top}\bfB_i^{*} = \mathbf{I}_{k\times k}$
	\end{itemize}
	
	
	
	
	
	
		
	
	
	
	

	
	
	
	



	
	
	
}

==> p2_low-dim-rep.tex <==






